Physics-Grounded Disentangled Flow Modeling for Brain Disease Progression Trajectory

Forecasting longitudinal brain lesion evolution is critical for disease monitoring and treatment planning. Existing approaches typically learn a direct mapping from a baseline image to a future observation, without explicitly modeling the physical mechanisms underlying the lesion progression. Such an entangled modeling of structural deformation and image intensity variation limits physical plausibility, model generalization, and interpretability. To address this, we propose PDF, a Physics-grounded Disentangled Flow matching framework for longitudinal brain disease forecasting. We explicitly decompose the longitudinal modeling of lesion growth into two processes, each learned by a dedicated flow matching network: morphology evolution, which captures lesion growth and structural deformation; and intensity evolution, which models signal changes driven by variations in lesion concentration. To enforce physics-grounded constraints, we introduce a PDE-regularized loss based on lesion growth dynamics, that enforces a diffusion-reaction-advection formulation for morphological evolution. Experiments on three public longitudinal datasets spanning diverse brain diseases demonstrate state-of-the-art performance, validating the effectiveness of the disentangled modeling framework and physics-grounded learning design. Code is publicly available at https://github.com/jhuldr/PDF.

==> tab_tex/eccv_comparison_table.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{makecell}
% \usepackage{graphicx}

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{1.35mm}
\renewcommand{\arraystretch}{1.15}
\fontsize{8.2}{9.6}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{l ccccc c ccccc c ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multicolumn{5}{c}{\textbf{UCSF (Tumor)}} &&
\multicolumn{5}{c}{\textbf{LUMIERE (Tumor)}} &&
\multicolumn{5}{c}{\textbf{LMSLS (MS)}} \\
\cmidrule(lr){2-6}
\cmidrule(lr){8-12}
\cmidrule(lr){14-18}
& \textbf{DSC}$\uparrow$
& \textbf{HD}$\downarrow$
& \textbf{PSNR}$\uparrow$
& \textbf{SSIM}$\uparrow$
& \textbf{L1}$\downarrow$
&& \textbf{DSC}$\uparrow$
& \textbf{HD}$\downarrow$
& \textbf{PSNR}$\uparrow$
& \textbf{SSIM}$\uparrow$
& \textbf{L1}$\downarrow$
&& \textbf{DSC}$\uparrow$
& \textbf{HD}$\downarrow$
& \textbf{PSNR}$\uparrow$
& \textbf{SSIM}$\uparrow$
& \textbf{L1}$\downarrow$ \\
\midrule

T-UNet~\cite{ronneberger2015u}
& \makecell{$0.728$\\{\scriptsize$\pm0.004$}}
& \makecell{$27.322$\\{\scriptsize$\pm0.812$}}
& \makecell{$\mathbf{31.739}$\\{\scriptsize$\pm0.103$}}
& \makecell{$0.920$\\{\scriptsize$\pm0.002$}}
& \makecell{$0.085$\\{\scriptsize$\pm0.002$}}
&& \makecell{$0.520$\\{\scriptsize$\pm0.020$}}
& \makecell{$38.135$\\{\scriptsize$\pm1.925$}}
& \makecell{$36.753$\\{\scriptsize$\pm0.185$}}
& \makecell{$0.845$\\{\scriptsize$\pm0.004$}}
& \makecell{$0.097$\\{\scriptsize$\pm0.003$}}
&& \makecell{$0.673$\\{\scriptsize$\pm0.005$}}
& \makecell{$26.354$\\{\scriptsize$\pm0.932$}}
& \makecell{$29.248$\\{\scriptsize$\pm0.118$}}
& \makecell{$0.805$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.083$\\{\scriptsize$\pm0.002$}} \\

I$^2$SB~\cite{liu2023i2sb}
& \makecell{$0.725$\\{\scriptsize$\pm0.005$}}
& \makecell{$28.839$\\{\scriptsize$\pm0.941$}}
& \makecell{$31.393$\\{\scriptsize$\pm0.097$}}
& \makecell{$0.920$\\{\scriptsize$\pm0.002$}}
& \makecell{$0.093$\\{\scriptsize$\pm0.002$}}
&& \makecell{$0.522$\\{\scriptsize$\pm0.035$}}
& \makecell{$36.105$\\{\scriptsize$\pm1.720$}}
& \makecell{$37.206$\\{\scriptsize$\pm0.348$}}
& \makecell{$0.953$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.084$\\{\scriptsize$\pm0.003$}}
&& \makecell{$0.682$\\{\scriptsize$\pm0.006$}}
& \makecell{$23.617$\\{\scriptsize$\pm0.784$}}
& \makecell{$29.312$\\{\scriptsize$\pm0.094$}}
& \makecell{$0.893$\\{\scriptsize$\pm0.002$}}
& \makecell{$0.068$\\{\scriptsize$\pm0.003$}} \\

TFM~\cite{zhang2024tfm}
& \makecell{$0.696$\\{\scriptsize$\pm0.006$}}
& \makecell{$31.701$\\{\scriptsize$\pm1.284$}}
& \makecell{$30.659$\\{\scriptsize$\pm0.125$}}
& \makecell{$0.898$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.091$\\{\scriptsize$\pm0.002$}}
&& \makecell{$0.492$\\{\scriptsize$\pm0.015$}}
& \makecell{$39.211$\\{\scriptsize$\pm1.530$}}
& \makecell{$36.317$\\{\scriptsize$\pm0.406$}}
& \makecell{$0.894$\\{\scriptsize$\pm0.001$}}
& \makecell{$0.088$\\{\scriptsize$\pm0.002$}}
&& \makecell{$0.670$\\{\scriptsize$\pm0.007$}}
& \makecell{$24.438$\\{\scriptsize$\pm0.851$}}
& \makecell{$\mathbf{29.441}$\\{\scriptsize$\pm0.102$}}
& \makecell{$0.889$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.062$\\{\scriptsize$\pm0.004$}} \\

ImageFlowNet~\cite{liu2025imageflownet}
& \makecell{$0.724$\\{\scriptsize$\pm0.004$}}
& \makecell{$28.402$\\{\scriptsize$\pm0.893$}}
& \makecell{$31.675$\\{\scriptsize$\pm0.108$}}
& \makecell{$0.909$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.085$\\{\scriptsize$\pm0.002$}}
&& \makecell{$0.493$\\{\scriptsize$\pm0.033$}}
& \makecell{$41.994$\\{\scriptsize$\pm1.653$}}
& \makecell{$37.178$\\{\scriptsize$\pm0.346$}}
& \makecell{$0.916$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.078$\\{\scriptsize$\pm0.003$}}
&& \makecell{$0.687$\\{\scriptsize$\pm0.005$}}
& \makecell{$24.296$\\{\scriptsize$\pm0.741$}}
& \makecell{$28.972$\\{\scriptsize$\pm0.113$}}
& \makecell{$0.890$\\{\scriptsize$\pm0.003$}}
& \makecell{$0.072$\\{\scriptsize$\pm0.002$}} \\

\textbf{PDF (Ours)}
& \makecell{$\mathbf{0.752}$\\{\scriptsize$\pm0.003$}}
& \makecell{$\mathbf{25.952}$\\{\scriptsize$\pm0.654$}}
& \makecell{$31.364$\\{\scriptsize$\pm0.092$}}
& \makecell{$\mathbf{0.920}$\\{\scriptsize$\pm0.001$}}
& \makecell{$\mathbf{0.072}$\\{\scriptsize$\pm0.002$}}
&& \makecell{$\mathbf{0.534}$\\{\scriptsize$\pm0.013$}}
& \makecell{$\mathbf{33.672}$\\{\scriptsize$\pm1.229$}}
& \makecell{$\mathbf{37.216}$\\{\scriptsize$\pm0.349$}}
& \makecell{$\mathbf{0.957}$\\{\scriptsize$\pm0.002$}}
& \makecell{$\mathbf{0.071}$\\{\scriptsize$\pm0.002$}}
&& \makecell{$\mathbf{0.696}$\\{\scriptsize$\pm0.004$}}
& \makecell{$\mathbf{20.867}$\\{\scriptsize$\pm0.623$}}
& \makecell{$29.314$\\{\scriptsize$\pm0.087$}}
& \makecell{$\mathbf{0.900}$\\{\scriptsize$\pm0.002$}}
& \makecell{$\mathbf{0.058}$\\{\scriptsize$\pm0.002$}} \\

\bottomrule
\end{tabular}%
}
\vspace{0.15cm}
\caption{\textbf{Quantitative comparison across three longitudinal datasets.} Mean $\pm$ standard deviation is reported. L1 denotes the image-level reconstruction error.}
\label{tab:comparison}
\vspace{-0.35cm}
\end{table*}

